Security of GPS/INS based On-road Location Tracking Systems

Location information is critical to a wide-variety of navigation and tracking applications. Today, GPS is the de-facto outdoor localization system but has been shown to be vulnerable to signal spoofing attacks. Inertial Navigation Systems (INS) are emerging as a popular complementary system, especially in road transportation systems as they enable improved navigation and tracking as well as offer resilience to wireless signals spoofing, and jamming attacks. In this paper, we evaluate the security guarantees of INS-aided GPS tracking and navigation for road transportation systems. We consider an adversary required to travel from a source location to a destination, and monitored by a INS-aided GPS system. The goal of the adversary is to travel to alternate locations without being detected. We developed and evaluated algorithms that achieve such goal, providing the adversary significant latitude. Our algorithms build a graph model for a given road network and enable us to derive potential destinations an attacker can reach without raising alarms even with the INS-aided GPS tracking and navigation system. The algorithms render the gyroscope and accelerometer sensors useless as they generate road trajectories indistinguishable from plausible paths (both in terms of turn angles and roads curvature). We also designed, built, and demonstrated that the magnetometer can be actively spoofed using a combination of carefully controlled coils. We implemented and evaluated the impact of the attack using both real-world and simulated driving traces in more than 10 cities located around the world. Our evaluations show that it is possible for an attacker to reach destinations that are as far as 30 km away from the true destination without being detected. We also show that it is possible for the adversary to reach almost 60-80% of possible points within the target region in some cities.

==> evaluation/impact.tex <==
\subsubsection*{\textbf{Impact of Algorithm Parameters}}

\input{evaluation/radius_impact}

\input{evaluation/sensor_impact}



==> evaluation/radius_impact.tex <==
\paragraph{Varying Radius of Coverage}

\begin{figure}[t]
	\centering
	\begin{subfigure}{.5\linewidth}
        \centering
		\includegraphics[width=\textwidth]{figures/parameters/All_Coverage_Radius_Impact_Mean.pdf}
		\caption{\label{fig:radius_impact_mean} Mean of Coverage Areas}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
        \centering
		\includegraphics[width=\textwidth]{figures/parameters/All_Coverage_Radius_Impact_Median.pdf}
		\caption{\label{fig:radius_impact_median} Median of Coverage Areas}
    \end{subfigure}
	\caption{Add Caption.}
	\label{fig:radius_impact}
\end{figure}

